Leveraging the Hankel norm approximation and block-AAA algorithms in reduced order modeling

Large-scale linear, time-invariant (LTI) dynamical systems are widely used to characterize complicated physical phenomena. We propose a two-stage algorithm to reduce the order of a large-scale LTI system given samples of its transfer function for a target degree $k$ of the reduced system. In the first stage, a modified adaptive Antoulas--Anderson (AAA) algorithm is used to construct a degree $d$ rational approximation of the transfer function that corresponds to an intermediate system, which can be numerically stably reduced in the second stage using ideas from the theory on Hankel norm approximation (HNA). We also study the numerical issues of Glover's HNA algorithm and provide a remedy for its numerical instabilities. A carefully computed rational approximation of degree $d$ gives us a numerically stable algorithm for reducing an LTI system, which is more efficient than SVD-based algorithms and more accurate than moment-matching algorithms.

==> macros.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,enumerate,enumitem,hyperref,cancel,xcolor,array,tabularx,bbm,esint,cleveref,stackengine,overpic,caption,rotating}
\usepackage[caption=false]{subfig} % <- Preamble
\usepackage{listings}% http://ctan.org/pkg/listings
\lstset{
  basicstyle=\ttfamily,
  mathescape
}
\usepackage[mathscr]{euscript}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{problem}{Problem}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

\newcommand{\pair}[2]{\left\langle #1, #2 \right\rangle_\mathbf{c}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\sS}{\mathbb{S}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\LTB}{\underline{\tilde{L}}}
\newcommand{\LB}{\underline{L}}
\newcommand{\XB}{\underline{X}}
\newcommand{\muB}{\underline{\mu}}
\newcommand{\cmax}{c_{\text{max}}}
\newcommand{\cmin}{c_{\text{min}}}
\DeclareMathOperator{\Ker}{Ker}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normc}[1]{\left\lVert#1\right\rVert_{\mathbf{c}}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\ceil}[1]{\lceil#1\rceil}
\DeclareMathOperator{\diff}{diff}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\aut}{Aut}
\newcommand{\comment}[1]{}

% Sets running headers as well as PDF title and authors
\headers{Leveraging the HNA and block-AAA algorithms in ROM}{A. Yu and A. Townsend}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Leveraging the Hankel norm approximation and block-AAA algorithms in reduced order modeling\thanks{xxx}}

% Authors: full names plus addresses.
\author{Annan Yu\thanks{Center for Applied Mathematics, Cornell University, Ithaca, 14853, NY, USA (\email{ay262@cornell.edu}).}
\and Alex Townsend\thanks{Department of Mathematics, Cornell University, Ithaca, 14853, NY, USA 
  (\email{townsend@cornell.edu}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Iner}{In}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows,positioning}

\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=1.2cm, 
minimum height=0.8cm, text centered, 
draw=black, fill=blue!30]

\tikzstyle{process} = [rectangle, 
minimum width=2cm, 
minimum height=1.2cm, 
text centered, 
text width=2cm, 
draw=black, 
fill=orange!30]

\tikzstyle{decision} = [diamond, 
minimum width=0.5cm, 
minimum height=0.5cm, 
text centered, 
draw=black, 
fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

